Channel Models for Multi-Level Cell Flash Memories Based on Empirical Error Analysis

We propose binary discrete parametric channel models for multi-level cell (MLC) flash memories that provide accurate ECC performance estimation by modeling the empirically observed error characteristics under program/erase (P/E) cycling stress. Through a detailed empirical error characterization of 1X-nm and 2Y-nm MLC flash memory chips from two different vendors, we observe and characterize the overdispersion phenomenon in the number of bit errors per ECC frame. A well studied channel model such as the binary asymmetric channel (BAC) model is unable to provide accurate ECC performance estimation. Hence we propose a channel model based on the beta-binomial probability distribution (2-BBM channel model) which is a good fit for the overdispersed empirical error characteristics and show through statistical tests and simulation results for BCH, LDPC and polar codes, that the 2-BBM channel model provides accurate ECC performance estimation in MLC flash memories.

==> tikz/2_bac.tex <==
	\begin{tikzpicture}[yscale=0.2, xscale=1.0, node distance=0.2cm, auto, thick]

	\draw[-, thick] (-1.0, 0.0) -- (1.0, 0.0);
	\draw[-, thick] (-1.0, -5.0) -- (1.0, -5.0);
	\draw[-, thick] (-1.0, 0.0) -- (1.0, -5.0);
	\draw[-, thick] (-1.0, -5.0) -- (1.0, 0.0);

	\node at (0.0, 1.0) {\scriptsize{$1 - p^{(u)}_{0}$}};
	\node at (0.0, -6.0) {\scriptsize{$1 - p^{(u)}_{1}$}};
	\node at (-0.1, -1.0) {\scriptsize{$p^{(u)}_{0}$}};
	\node at (-0.2, -4.0) {\scriptsize{$p^{(u)}_{1}$}};

	\node at (-1.1, 0.0) {\scriptsize{0}};
	\node at (-1.1, -5.0) {\scriptsize{1}};
	\node at (1.1, 0.0) {\scriptsize{0}};
	\node at (1.1, -5.0) {\scriptsize{1}};

	\draw[-] (-1.0, -10.0) -- (1.0, -10.0);
	\draw[-] (-1.0, -15.0) -- (1.0, -15.0);
	\draw[-] (-1.0, -10.0) -- (1.0, -15.0);
	\draw[-] (-1.0, -15.0) -- (1.0, -10.0);

	\node at (0.0, -9.0) {\scriptsize{$1 - p^{(l)}_{0}$}};
	\node at (0.0, -16.0) {\scriptsize{$1 - p^{(l)}_{1}$}};
	\node at (-0.1, -11.0) {\scriptsize{$p^{(l)}_{0}$}};
	\node at (-0.2, -14.0) {\scriptsize{$p^{(l)}_{1}$}};

	\node at (-1.1, -10.0) {\scriptsize{0}};
	\node at (-1.1, -15.0) {\scriptsize{1}};
	\node at (1.1, -10.0) {\scriptsize{0}};
	\node at (1.1, -15.0) {\scriptsize{1}};

	\draw [dashed] (-1.5, 2.0) rectangle (1.5, -7.0);
	\draw [dashed] (-1.5, -8.0) rectangle (1.5, -17.0);

	\node at (0.0, 3.0) {\scriptsize{Upper Page BAC}};
	\node at (0.0, -18.0) {\scriptsize{Lower Page BAC}};



	\node at (-2.5, -2.5) {$x^{(u)}$};
	\node at (-2.5, -12.5) {$x^{(l)}$};
	\draw[->, thick] (-2.2, -2.7) -- (-1.5, -2.7);
	\draw[->, thick] (-2.2, -12.7) -- (-1.5, -12.7);
	\draw[-, thick] (-3.2, -2.7) -- (-2.8, -2.7);
	\draw[-, thick] (-3.2, -12.7) -- (-2.8, -12.7);
	\draw[-, thick] (-3.2, -2.7) -- (-3.2, -12.7);
	\draw[->, thick] (-4.0, -7.7) -- (-3.2, -7.7);
	\node at (-4.2, -7.7) {$x$};

	\node at (2.5, -2.5) {$y^{(u)}$};
	\node at (2.5, -12.5) {$y^{(l)}$};
	\draw[->, thick] (1.5, -2.7) -- (2.2, -2.7);
	\draw[->, thick] (1.5, -12.7) -- (2.2, -12.7);
	\draw[-, thick] (2.8, -2.7) -- (3.2, -2.7);
	\draw[-, thick] (2.8, -12.7) -- (3.2, -12.7);
	\draw[-, thick] (3.2, -2.7) -- (3.2, -12.7);
	\draw[->, thick] (3.2, -7.7) -- (4.0, -7.7);
	\node at (4.2, -7.7) {$y$};

	\draw [-, thick] (-3.6, 4.0) rectangle (3.6, -19.0);

	\end{tikzpicture}


==> tikz/2_bsc.tex <==
\begin{tikzpicture}[yscale=0.2, xscale=1.0, node distance=0.2cm, auto, thick]
	
	\draw[-, thick] (-1.0, 0.0) -- (1.0, 0.0);
	\draw[-, thick] (-1.0, -5.0) -- (1.0, -5.0);
	\draw[-, thick] (-1.0, 0.0) -- (1.0, -5.0);
	\draw[-, thick] (-1.0, -5.0) -- (1.0, 0.0);
	
	\node at (0.0, 1.0) {\scriptsize{$1 - p^{(l)}$}};
	\node at (0.0, -6.0) {\scriptsize{$1 - p^{(l)}$}};
	\node at (-0.1, -1.0) {\scriptsize{$p^{(l)}$}};
	\node at (-0.2, -4.0) {\scriptsize{$p^{(l)}$}};
	
	\node at (-1.1, 0.0) {\scriptsize{0}};
	\node at (-1.1, -5.0) {\scriptsize{1}};
	\node at (1.1, 0.0) {\scriptsize{0}};
	\node at (1.1, -5.0) {\scriptsize{1}};
	
	\draw[-] (-1.0, -10.0) -- (1.0, -10.0);
	\draw[-] (-1.0, -15.0) -- (1.0, -15.0);
	\draw[-] (-1.0, -10.0) -- (1.0, -15.0);
	\draw[-] (-1.0, -15.0) -- (1.0, -10.0);
	
	\node at (0.0, -9.0) {\scriptsize{$1 - p^{(u)}$}};
	\node at (0.0, -16.0) {\scriptsize{$1 - p^{(u)}$}};
	\node at (-0.1, -11.0) {\scriptsize{$p^{(u)}$}};
	\node at (-0.2, -14.0) {\scriptsize{$p^{(u)}$}};
	
	\node at (-1.1, -10.0) {\scriptsize{0}};
	\node at (-1.1, -15.0) {\scriptsize{1}};
	\node at (1.1, -10.0) {\scriptsize{0}};
	\node at (1.1, -15.0) {\scriptsize{1}};
	
	\draw [dashed] (-1.5, 2.0) rectangle (1.5, -7.0);
	\draw [dashed] (-1.5, -8.0) rectangle (1.5, -17.0);
	
	\node at (0.0, 3.0) {\scriptsize{Lower Page}};
	\node at (0.0, -18.0) {\scriptsize{Upper Page}};
	
	
	
	\node at (-2.5, -2.5) {$x^{(l)}$};
	\node at (-2.5, -12.5) {$x^{(u)}$};
	\draw[->, thick] (-2.2, -2.7) -- (-1.5, -2.7);
	\draw[->, thick] (-2.2, -12.7) -- (-1.5, -12.7);
	\draw[-, thick] (-3.2, -2.7) -- (-2.8, -2.7);
	\draw[-, thick] (-3.2, -12.7) -- (-2.8, -12.7);
	\draw[-, thick] (-3.2, -2.7) -- (-3.2, -12.7);
	\draw[->, thick] (-4.0, -7.7) -- (-3.2, -7.7);
	\node at (-4.2, -7.7) {$x$};
	
	\node at (2.5, -2.5) {$y^{(l)}$};
	\node at (2.5, -12.5) {$y^{(u)}$};
	\draw[->, thick] (1.5, -2.7) -- (2.2, -2.7);
	\draw[->, thick] (1.5, -12.7) -- (2.2, -12.7);
	\draw[-, thick] (2.8, -2.7) -- (3.2, -2.7);
	\draw[-, thick] (2.8, -12.7) -- (3.2, -12.7);
	\draw[-, thick] (3.2, -2.7) -- (3.2, -12.7);
	\draw[->, thick] (3.2, -7.7) -- (4.0, -7.7);
	\node at (4.2, -7.7) {$y$};
	
	\draw [-, thick] (-3.6, 4.0) rectangle (3.6, -19.0);
	
	\end{tikzpicture}

==> tikz/4_dmc.tex <==

\begin{tikzpicture}[yscale=0.2, xscale=1.0, node distance=0.2cm, auto, thick]

\draw[-, thick] (-1.0, 0.0) -- (1.0, 0.0);
\draw[-, thick] (-1.0, 0.0) -- (1.0, -5.0);
\draw[-, thick] (-1.0, 0.0) -- (1.0, -10.0);
\draw[-, thick] (-1.0, 0.0) -- (1.0, -15.0);

\draw[-, thick] (-1.0, -5.0) -- (1.0, 0.0);
\draw[-, thick] (-1.0, -5.0) -- (1.0, -5.0);
\draw[-, thick] (-1.0, -5.0) -- (1.0, -10.0);
\draw[-, thick] (-1.0, -5.0) -- (1.0, -15.0);

\draw[-, thick] (-1.0, -10.0) -- (1.0, -0.0);
\draw[-, thick] (-1.0, -10.0) -- (1.0, -5.0);
\draw[-, thick] (-1.0, -10.0) -- (1.0, -10.0);
\draw[-, thick] (-1.0, -10.0) -- (1.0, -15.0);


\draw[-, thick] (-1.0, -15.0) -- (1.0, 0.0);
\draw[-, thick] (-1.0, -15.0) -- (1.0, -5.0);
\draw[-, thick] (-1.0, -15.0) -- (1.0, -10.0);
\draw[-, thick] (-1.0, -15.0) -- (1.0, -15.0);

%\node at (0.0, 1.0) {\scriptsize{$1 - p^{(l)}_{0}$}};
%\node at (0.0, -6.0) {\scriptsize{$1 - p^{(l)}_{1}$}};
%\node at (-0.1, -1.0) {\scriptsize{$p^{(l)}_{0}$}};
%\node at (-0.2, -4.0) {\scriptsize{$p^{(l)}_{1}$}};

\node at (-1.4, 1.0) {\tiny{$p_{00}$}};
\node at (-1.4, 0.0) {\tiny{$p_{01}$}};
\node at (-1.4, -1.0) {\tiny{$p_{02}$}};
\node at (-1.4, -2.0) {\tiny{$p_{03}$}};

\node at (-1.4, -4.0) {\tiny{$p_{10}$}};
\node at (-1.4, -5.0) {\tiny{$p_{11}$}};
\node at (-1.4, -6.0) {\tiny{$p_{12}$}};
\node at (-1.4, -7.0) {\tiny{$p_{13}$}};

\node at (-1.4, -9.0) {\tiny{$p_{20}$}};
\node at (-1.4, -10.0) {\tiny{$p_{21}$}};
\node at (-1.4, -11.0) {\tiny{$p_{22}$}};
\node at (-1.4, -12.0) {\tiny{$p_{23}$}};

\node at (-1.4, -14.0) {\tiny{$p_{30}$}};
\node at (-1.4, -15.0) {\tiny{$p_{31}$}};
\node at (-1.4, -16.0) {\tiny{$p_{32}$}};
\node at (-1.4, -17.0) {\tiny{$p_{33}$}};

\node at (-1.1, 0.0) {\scriptsize{0}};
\node at (-1.1, -5.0) {\scriptsize{1}};
\node at (-1.1, -10.0) {\scriptsize{2}};
\node at (-1.1, -15.0) {\scriptsize{3}};

\node at (1.1, 0.0) {\scriptsize{0}};
\node at (1.1, -5.0) {\scriptsize{1}};
\node at (1.1, -10.0) {\scriptsize{2}};
\node at (1.1, -15.0) {\scriptsize{3}};

\end{tikzpicture}

==> tikz/shift_read_model.tex <==
	\begin{tikzpicture}
	\begin{groupplot}[
	group style={
		group name=my plots,
		group size=1 by 1,
		ylabels at=edge left
	},
	no markers,
	xmin=0,xmax=8,
	%domain=-1:8,
	%samples=150,
	footnotesize,
	width=16cm,
	height=5cm,
	tickpos=left,
	%ytick align=outside,
	xtick=\empty,
	ytick=\empty,
	x label style={at={(axis description cs:0.7,-0.1)},anchor=north},
    y label style={at={(axis description cs:0.13,0.9)},anchor=south},
	xlabel={Threshold voltage},
	ylabel={Number of flash memory cells},
	%xtick align=outside,
	clip=false, axis on top,
	axis lines*=left,
	enlargelimits=false
	]

	\nextgroupplot
	\addplot [domain=0:2, samples=50, thick] {gauss(1,0.25)};
	\addplot [domain=2:4, samples=50, thick] {gauss(3,0.25)};
	\addplot [domain=4:6, samples=50, thick] {gauss(5,0.25)};
	\addplot [domain=6:8, samples=50, thick] {gauss(7,0.25)};
	%\addplot [very thick,cyan!50!black] {gauss(6.5,1)};

	\node at (axis cs:1,1.7) [anchor=south] {E(0)};
	\node at (axis cs:3,1.7) [anchor=south] {A(1)};
	\node at (axis cs:5,1.7) [anchor=south] {B(2)};
	\node at (axis cs:7,1.7) [anchor=south] {C(3)};
	\node at (axis cs:2.0,0) [anchor=north] {$V_A$};
	\draw[-, dashed, thick] (axis cs:2.0,0) -- (axis cs:2.0,2.0);
	\draw[-, dashed, thick] (axis cs:2.2,0) -- (axis cs:2.2,2.0);
	\draw[-, dashed, thick] (axis cs:1.8,0) -- (axis cs:1.8,2.0);
	\draw[-, dashed, thick] (axis cs:2.4,0) -- (axis cs:2.4,2.0);
	\draw[-, dashed, thick] (axis cs:1.6,0) -- (axis cs:1.6,2.0);
	\draw[-, dashed, thick] (axis cs:2.6,0) -- (axis cs:2.6,2.0);
	\draw[-, dashed, thick] (axis cs:1.4,0) -- (axis cs:1.4,2.0);

	\node at (axis cs:4.0,0) [anchor=north] {$V_B$};
	\draw[-, dashed, thick] (axis cs:4.0,0) -- (axis cs:4.0,2.0);
	\draw[-, dashed, thick] (axis cs:4.2,0) -- (axis cs:4.2,2.0);
	\draw[-, dashed, thick] (axis cs:3.8,0) -- (axis cs:3.8,2.0);
	\draw[-, dashed, thick] (axis cs:4.4,0) -- (axis cs:4.4,2.0);
	\draw[-, dashed, thick] (axis cs:3.6,0) -- (axis cs:3.6,2.0);
	\draw[-, dashed, thick] (axis cs:4.6,0) -- (axis cs:4.6,2.0);
	\draw[-, dashed, thick] (axis cs:3.4,0) -- (axis cs:3.4,2.0);

	\node at (axis cs:6.0,0) [anchor=north] {$V_C$};
	\draw[-, dashed, thick] (axis cs:6.0,0) -- (axis cs:6.0,2.0);
	\draw[-, dashed, thick] (axis cs:6.2,0) -- (axis cs:6.2,2.0);
	\draw[-, dashed, thick] (axis cs:5.8,0) -- (axis cs:5.8,2.0);
	\draw[-, dashed, thick] (axis cs:6.4,0) -- (axis cs:6.4,2.0);
	\draw[-, dashed, thick] (axis cs:5.6,0) -- (axis cs:5.6,2.0);
	\draw[-, dashed, thick] (axis cs:6.6,0) -- (axis cs:6.6,2.0);
	\draw[-, dashed, thick] (axis cs:5.4,0) -- (axis cs:5.4,2.0);

	\node at (axis cs:1.0,0.0) [anchor=north] {11};
	\node at (axis cs:3.0,0.0) [anchor=north] {10};
	\node at (axis cs:5.0,0.0) [anchor=north] {00};
	\node at (axis cs:7.0,0.0) [anchor=north] {01};

	\draw [thick, decoration={brace, amplitude=8pt, raise=0.5cm}, decorate] (axis cs:1.4,1.8) -- (axis cs:2.6,1.8);
	\draw [thick, decoration={brace, amplitude=8pt, raise=0.5cm}, decorate] (axis cs:3.4,1.8) -- (axis cs:4.6,1.8);
	\draw [thick, decoration={brace, amplitude=8pt, raise=0.5cm}, decorate] (axis cs:5.4,1.8) -- (axis cs:6.6,1.8);

	\node at (axis cs:2.0,2.6) [anchor=north] {$r$ reads};
	\node at (axis cs:4.0,2.6) [anchor=north] {$r$ reads};
	\node at (axis cs:6.0,2.6) [anchor=north] {$r$ reads};


	\end{groupplot}
	\end{tikzpicture}

